Multi-Dimensional Evaluation of Text Summarization with In-Context Learning

Evaluation of natural language generation (NLG) is complex and multi-dimensional. Generated text can be evaluated for fluency, coherence, factuality, or any other dimensions of interest. Most frameworks that perform such multi-dimensional evaluation require training on large manually or synthetically generated datasets. In this paper, we study the efficacy of large language models as multi-dimensional evaluators using in-context learning, obviating the need for large training datasets. Our experiments show that in-context learning-based evaluators are competitive with learned evaluation frameworks for the task of text summarization, establishing state-of-the-art on dimensions such as relevance and factual consistency. We then analyze the effects of factors such as the selection and number of in-context examples on performance. Finally, we study the efficacy of in-context learning based evaluators in evaluating zero-shot summaries written by large language models such as GPT-3.

==> sections/related.tex <==
\section{Related Work} \label{related}
Some of the most commonly used automatic evaluation metrics rely on n-gram overlaps between the generated text and a reference text \cite{papineni-2002-bleu, lin-2004-rouge}. These metrics are easy to use but often do not correlate well with human evaluations, especially as generation systems themselves have become increasingly sophisticated and less amenable to evaluation on the basis of surface level features. Reference-based learned metrics \cite{sellam-2020-bleurt, zhao-2019-moverscore, zhang-2020-bertscore} attempt to alleviate some of these issues by injecting learned components such as contextual representations within the evaluation pipeline. 

The drawbacks of the single-score metrics such as the ones mentioned above include insufficiency to comprehensively evaluate generated text and the lack of human interpretability. This has prompted work proposing evaluators for specific human-interpretable and task-specific aspects, such as consistency in summarization \cite{kryscinski-2020-evaluating, wang-2020-asking} and coherence in dialog response generation \cite{dziri-2019-evaluating, huang-2020-grade}. 

Consequently, recent work has proposed evaluation frameworks for simultaneously evaluating on multiple human-evaluation criteria. This is achieved by modifying formulas within a broader common framework \cite{deng-2021-compression} or by selecting different inputs or outputs, such as source or reference texts, to give scores aligned to different aspects \cite{yuan-2021-bartscore}. More recently, \cite{zhong-2022-towards} propose the UniEval framework that formulates evaluation as a boolean question-answering task and train an evaluator using multi-task and continual learning for multiple aspects, such that the model can evaluate each of the trained aspects by changing the question being asked. For example, the question \textit{"Is this a coherent summary to the document?"} would evaluate a given summary on coherence. Our work is most similar in spirit to UniEval, but instead of fine-tuning a pre-trained encoder-decoder model, we rely on an in-context learning backbone that allows us to leverage powerful autoregressive models such as GPT-3 to perform few-shot evaluation, in contrast with previous evaluation frameworks that rely on fine-tuning on much larger datasets.
